WiSleep: Inferring Sleep Duration at Scale Using Passive WiFi Sensing

Sleep deprivation is a public health concern that significantly impacts one's well-being and performance. Sleep is an intimate experience, and state-of-the-art sleep monitoring solutions are highly-personalized to individual users. With a motivation to expand sleep monitoring capabilities at a large scale and contribute sleep data to public health understanding, we present Wisleep, a system for inferring sleep duration using smartphone network connections that are passively sensed from WiFi infrastructure. We propose an unsupervised ensemble model of Bayesian change point detection, validating it over a user study among 20 students living in campus dormitories and a private home. Our results find Wisleep outperforming prior techniques for users with irregular sleep patterns while yielding an average 88.50% accuracy within 60 minutes sleep time error and 39 minutes wake-up time error. This is comparable to client-side methods, albeit utilizing coarse-grained information. Additionally, we utilize our approach to predict sleep and wake-up times from a user study of more than 1000 student users, demonstrating results similar to prior findings on students' sleep patterns. Finally, we show that Wisleep can process data from twenty thousand users on a single commodity server, allowing it to scale to large campus populations with low server requirements.

==> Data.tex <==


\subsection{Ground Truth Labels}
\begin{enumerate}
    \item For validation: logs of 5 users 
    \item ...We also looked for evidence of polyphasic sleep schedules and disturbed cycles that are common among students and unfortunately, might be associated with or increase the risk of poor sleep. 
    \item interrater reliability on manual labels
\end{enumerate}
 
\subsection{WiFi Activity Data}
\begin{enumerate}
    \item describe wifi data, relevant fields. 
    \item how much data did you work with? Any pre-processing steps?
    \item 
\end{enumerate}
